Challenges in Finding Stable Price Zones in European Electricity Markets: Aiming to Square the Circle?

The European day-ahead electricity market is split into multiple bidding zones with a uniform price. The increase in renewables leads to a growing number of interventions in the generation of energy sources and increasing redispatch costs. To ensure efficient congestion management, the EU Commission mandated a Bidding Zone Review (BZR) to reevaluate the configuration of European bidding zones. An integral part of this process was a locational marginal pricing study. Based on these prices, alternative bidding zone configurations were proposed. These bidding zones shall be stable and robust over time. For Germany, four configurations were suggested. We analyzed the proposed configurations considering different clustering algorithms and periods based on the publicly released data set in the context of the BZR, and found that the configurations do not reduce the price standard deviations within zones much, and the average prices across zones are similar. Other configurations identified based on clustering the prices lead to lower price variance but they are not geographically coherent. Independent of the clustering features and algorithms used, the resulting clusters are not stable over time. Interestingly, the effect of a split on prices would be low based on an analysis of the BZR data set.

==> cluster_price_analysis.tex <==
\section{Cluster price analysis for the alternative configurations proposed by ACER} \label{app:cluster-price-analysis}

\subsection{Cluster price standard deviations} \label{app:cluster-variances}

Table \ref{tab:price-std-summary} shows the average price standard deviations of a single price zone configuration as well as of the configurations proposed by ACER.

\begin{table}[!htp]
    \centering
    \begin{tabular}{c|c|c|c}
        & 1989 & 1995 & 2009 \\
        \hline
        Single price zone & 14.54 & 14.32 & 11.48 \\
        DE2 (k-means) & 13.09 & 12.93 & 10.85 \\ 
        DE2 (spectral) & 13.98 & 13.80 & 11.22 \\
        DE3 (spectral) & 13.86 & 13.65 & 11.26 \\
        DE4 (spectral) & 13.14 & 13.02 & 10.87 \\
    \end{tabular}
    \caption{Average price standard deviations of configurations with 1, 2, 3 or 4 price zones}
    \label{tab:price-std-summary}
\end{table}

The following plots illustrate, for every configuration, the cluster price standard deviation corresponding to each week in \textcolor{blue}{the scenario years} 1989, 1995, and 2009. 
A point represents the price standard deviation of a specific cluster in a specific week. Depending on the configuration (i.e., number of clusters), multiple points are shown for the same week.
Figure \ref{fig:1-zone-price-var} highlights the weekly price standard deviation of a single price zone for each year we consider.

\begin{figure}[!htp]
	\centering
	\includegraphics[width=.32\textwidth]{figures/1_zone_std_1989.png}
	\includegraphics[width=.32\textwidth]{figures/1_zone_std_1995.png}
	\includegraphics[width=.32\textwidth]{figures/1_zone_std_2009.png}
	\caption{Single price zone (cluster)}
	\label{fig:1-zone-price-var}

	\centering
	\includegraphics[width=.32\textwidth]{figures/DE2(k-means)_std_1989.png}
	\includegraphics[width=.32\textwidth]{figures/DE2(k-means)_std_1995.png}
	\includegraphics[width=.32\textwidth]{figures/DE2(k-means)_std_2009.png}
	\caption{DE2 (k-means)}
	\label{fig:de2-kmeans-price-var}
\end{figure}

\begin{figure}[!htp]
	\centering
	\includegraphics[width=.32\textwidth]{figures/DE2(spectral)_std_1989.png}
	\includegraphics[width=.32\textwidth]{figures/DE2(spectral)_std_1995.png}
	\includegraphics[width=.32\textwidth]{figures/DE2(spectral)_std_2009.png}
	\caption{DE2 (spectral)}
	\label{fig:de2-spectral-price-var}

	\centering
	\includegraphics[width=.32\textwidth]{figures/DE3(spectral)_std_1989.png}
	\includegraphics[width=.32\textwidth]{figures/DE3(spectral)_std_1995.png}
	\includegraphics[width=.32\textwidth]{figures/DE3(spectral)_std_2009.png}
	\caption{DE3 (spectral)}
	\label{fig:de3-spectral-price-var}

    % \vspace{1.5cm}
	
    \centering
	\includegraphics[width=.32\textwidth]{figures/DE4(spectral)_std_1989.png}
	\includegraphics[width=.32\textwidth]{figures/DE4(spectral)_std_1995.png}
	\includegraphics[width=.32\textwidth]{figures/DE4(spectral)_std_2009.png}
	\caption{DE4 (spectral)}
	\label{fig:de4-spectral-price-var}
\end{figure}


\newpage 

\subsection{Average cluster prices} \label{app:cluster-average-prices}

In the following tables, $\Delta^{\text{year}}_\mu$ represents the average distance between cluster mean prices for a specific year, i.e., $\Delta^{\text{year}}_\mu = \frac{1}{8} \displaystyle\sum_{i \in \{1, \dots, 8\}} \Delta^{\text{W}_i}_\mu$, where $\Delta^{\text{W}_i}_\mu$ is the average distance between cluster mean prices for week $\text{W}_i$ (see Section \ref{sec:intra-inter-similarity}).
\begin{table}[!htp]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c||c}
        & & W1 & W2 & W3 & W4 & W5 & W6 & W7 & W8 & $\Delta^{\text{year}}$ \\
        \hline
        1989 & Cluster 1 & 50.49 & 46.72 & 41.99 & 49.88 & 48.52 & 39.52 & 40.22 & 45.50 & - \\
        1995 & Cluster 1 & 39.87 & 28.09 & 45.89 & 46.11 & 48.61 & 38.35 & 51.76 & 54.50 & - \\
        2009 & Cluster 1 & 50.49 & 51.94 & 41.99 & 47.66 & 45.89 & 46.11 & 39.52 & 40.91 & - \\
    \end{tabular}
    \caption{Cluster average prices (EUR/MWh) - Single price zone (cluster)}
    \label{tab:average-prices-1-cluster}
 \end{table}


 \begin{table}[!htp]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c||c}
        & & W1 & W2 & W3 & W4 & W5 & W6 & W7 & W8 & $\Delta^{\text{year}}_\mu$ \\
        \hline
        \multirow{2}{*}{1989} & Cluster 1 & 49.09 & 45.71 & 39.18 & 49.32 & 47.94 & 35.84 & 37.44 & 44.38 & \multirow{2}{*}{4.3}  \\
        & Cluster 2 & 52.55 & 48.21 & 46.10 & 50.69 & 49.39 & 44.91 & 44.28 & 47.15 \\
        \hline

        \multirow{2}{*}{1995} & Cluster 1 & 35.02 & 21.21 & 44.56 & 45.13 & 47.65 & 35.63 & 51.22 & 54.14 & \multirow{2}{*}{5.75} \\
        & Cluster 2 & 46.98 & 38.19 & 47.84 & 47.55 & 50.03 & 42.35 & 52.56 & 55.04 \\
        \hline

        \multirow{2}{*}{2009} & Cluster 1 & 49.09 & 51.21 & 39.18 & 47.11 & 44.56 & 45.13 & 35.84 & 37.25 & \multirow{2}{*}{4.67} \\
        & Cluster 2 & 52.55 & 53.01 & 46.10 & 48.46 & 47.84 & 47.55 & 44.91 & 46.28 \\
    
    \end{tabular}
    \caption{Cluster average prices (EUR/MWh) - DE2 (k-means)}
    \label{tab:average-prices-DE2-kmeans}
 \end{table}


\begin{table}[!htp]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c||c}
        & & W1 & W2 & W3 & W4 & W5 & W6 & W7 & W8 & $\Delta^{\text{year}}_\mu$ \\
        \hline
        \multirow{2}{*}{1989} & Cluster 1 & 48.87 & 45.52 & 38.77 & 49.13 & 47.73 & 34.89 & 36.80 & 44.29 &  \multirow{2}{*}{4.17} \\
        & Cluster 2 & 52.07 & 47.90 & 45.14 & 50.61 & 49.31 & 44.05 & 43.56 & 46.70 \\
        \hline

        \multirow{2}{*}{1995} & Cluster 1 & 34.06 & 20.40 & 44.22 & 44.91 & 47.36 & 35.03 & 51.08 & 54.08 &  \multirow{2}{*}{5.46} \\
        & Cluster 2 & 45.56 & 35.63 & 47.53 & 47.29 & 49.84 & 41.61 & 52.44 & 54.91 \\
        \hline

        \multirow{2}{*}{2009} & Cluster 1 & 48.87 & 51.06 & 38.77 & 46.91 & 44.22 & 44.91 & 34.89 & 36.81 &  \multirow{2}{*}{4.47} \\
        & Cluster 2 & 52.07 & 52.80 & 45.14 & 48.39 & 47.53 & 47.29 & 44.05 & 44.93 \\
    \end{tabular}
    \caption{Cluster average prices (EUR/MWh) - DE2 (spectral)}
    \label{tab:average-prices-DE2-spectral}
 \end{table}


 \begin{table}[!htp]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c||c}
        & & W1 & W2 & W3 & W4 & W5 & W6 & W7 & W8 & $\Delta^{\text{year}}_\mu$  \\
        \hline
        \multirow{2}{*}{1989} & Cluster 1 & 52.68 & 48.38 & 46.38 & 50.72 & 49.36 & 44.96 & 44.58 & 47.43 &  \multirow{3}{*}{3.09} \\
        & Cluster 2 & 49.17 & 45.94 & 40.29 & 49.85 & 48.51 & 37.41 & 38.86 & 44.68 \\
        & Cluster 3 & 49.72 & 45.81 & 39.04 & 48.88 & 47.51 & 35.88 & 36.81 & 44.32 \\
        \hline

        \multirow{2}{*}{1995} & Cluster 1 & 47.30 & 38.88 & 47.80 & 47.66 & 50.05 & 42.57 & 52.58 & 55.08 & \multirow{3}{*}{3.99} \\
        & Cluster 2 & 36.69 & 23.49 & 45.31 & 45.88 & 48.37 & 36.26 & 51.77 & 54.24 \\
        & Cluster 3 & 35.34 & 21.51 & 44.37 & 44.53 & 47.18 & 36.21 & 50.73 & 54.18 \\
        \hline
        
        \multirow{2}{*}{2009} & Cluster 1 & 52.68 & 53.05 & 46.38 & 48.42 & 47.8 & 47.66 & 44.96 & 46.74 & \multirow{3}{*}{3.37} \\
        & Cluster 2 & 49.17 & 51.49 & 40.29 & 47.89 & 45.31 & 45.88 & 37.41 & 38.87 \\
        & Cluster 3 & 49.72 & 51.21 & 39.04 & 46.38 & 44.37 & 44.53 & 35.88 & 36.69 \\
    \end{tabular}
    \caption{Cluster average prices (EUR/MWh) - DE3 (spectral)}
    \label{tab:average-prices-DE3-spectral}

\vspace{1.5cm}

    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c||c}
        & & W1 & W2 & W3 & W4 & W5 & W6 & W7 & W8 & $\Delta^{\text{year}}_\mu$  \\
        \hline
        \multirow{4}{*}{1989} & Cluster 1 & 49.03 & 46.0 & 39.51 & 49.91 & 48.52 & 36.68 & 38.28 & 44.48 & \multirow{4}{*}{3.14} \\
        & Cluster 2 & 52.30 & 47.85 & 45.41 & 50.94 & 49.77 & 44.74 & 43.06 & 46.37 \\
        & Cluster 3 & 49.00 & 45.41 & 38.73 & 48.84 & 47.44 & 34.78 & 36.55 & 44.25 \\
        & Cluster 4 & 52.62 & 48.50 & 46.44 & 50.37 & 48.91 & 44.81 & 45.46 & 47.86 \\
        \hline
        
        \multirow{4}{*}{1995} & Cluster 1 & 35.24 & 21.24 & 44.78 & 45.75 & 48.32 & 36.11 & 51.63 & 54.13 & \multirow{4}{*}{4.19} \\
        & Cluster 2 & 45.35 & 35.98 & 47.97 & 47.80 & 50.53 & 41.13 & 53.33 & 55.07 \\
        & Cluster 3 & 34.37 & 20.74 & 44.23 & 44.60 & 47.05 & 34.99 & 50.87 & 54.11 \\
        & Cluster 4 & 48.32 & 39.51 & 47.58 & 47.13 & 49.35 & 43.53 & 51.58 & 54.94 \\
        \hline
        
        \multirow{4}{*}{2009} & Cluster 1 & 49.03 & 51.29 & 39.51 & 47.72 & 44.78 & 45.75 & 36.68 & 37.71 & \multirow{4}{*}{3.34} \\
         & Cluster 2 & 52.30 & 53.05 & 45.41 & 49.11 & 47.97 & 47.80 & 44.74 & 44.95 \\
         & Cluster 3 & 49.00 & 51.07 & 38.73 & 46.6 & 44.23 & 44.60 & 34.78 & 36.69 \\
         & Cluster 4 & 52.62 & 52.87 & 46.44 & 47.67 & 47.58 & 47.13 & 44.81 & 47.18 \\
    \end{tabular}
    \caption{Cluster average prices - DE4 (spectral)}
    \label{tab:average-prices-DE4-spectral}
 \end{table}


==> one_day_analysis.tex <==
\section{Single-day clustering analysis} \label{app:one-day-analysis}

The time granularity of the prices included in the clustering computation influences the stability of the resulting clusterings. 
In what follows, we analyze the stability of the clusterings identified given the prices corresponding to a single day.
We select the \textcolor{blue}{scenario} day of January 22, 1989, and compute clusterings using K-Means and Spectral Clustering.
As clustering feature(s), we consider (1) the time series of prices of a node (12 hours, i.e., 12 features) and (2) the time series of prices of a node and its geographic coordinates.

Table \ref{tab:one-day} shows the values of the inter- and intra-cluster similarity metrics introduced in Section \ref{sec:intra-inter-similarity}.
We observe the average distances between cluster mean prices ($\Delta_\mu$) and the average distances between all points situated in different clusters ($\Delta_{\text{avg}}$) are considerably lower compared to the values shown in Table \ref{tab:1}, indicating that the clusters are similar to each other and thus not well-defined.
We recall that the results illustrated in Table \ref{tab:1} correspond to clusterings obtained considering the annual time series of nodal prices as clustering features.
With time series of smaller length, clusterings appear to be less stable.

\begin{table}[!htp]
	\centering
	\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
		$k$ & Alg. & Loc. & $\sigma$ & $\Delta_\mu$ & $\Delta_\text{min}$ & $\Delta_\text{avg}$ & $DB$ & $\mu_1$ & $\mu_2$ & $\mu_3$ & $\mu_4$ \\
		\hline 
		2 & K-Means &  & 12.78 & 0.81 & 0.0 & 0.8 & 0.94 & 56.31 & 57.12 & - & - \\
        2 & K-Means & x & 16.17 & 0.39 & 0.0 & 0.56 & 2.03 & 56.35 & 56.74 & - & - \\
        2 & Spectral &  & 13.23 & 0.76 & 0.0 & 0.78 & 1.01 & 56.32 & 57.08 & - & - \\
        2 & Spectral & x & 11.28 & 0.33 & 0.0 & 0.39 & 0.73 & 56.43 & 56.1 & - & - \\
        \hline
        3 & K-Means &  & 11.16 & 0.73 & 0.09 & 0.75 & 0.83 & 56.34 & 56.07 & 57.17 & - \\
        3 & K-Means & x & 10.38 & 0.23 & 0.0 & 0.34 & 1.09 & 56.43 & 56.4 & 56.08 & - \\
        3 & Spectral &  & 12.62 & 0.77 & 0.0 & 0.78 & 1.04 & 56.36 & 57.13 & 55.97 & - \\
        3 & Spectral & x & 13.44 & 0.47 & 0.0 & 0.55 & 1.71 & 56.39 & 56.78 & 56.07 & - \\
        \hline
        4 & K-Means &  & 12.88 & 0.57 & 0.08 & 0.57 & 1.11 & 56.61 & 56.13 & 57.23 & 56.47 \\
        4 & K-Means & x & 12.94 & 0.3 & 0.0 & 0.39 & 5.21 & 56.68 & 56.08 & 56.35 & 56.33 \\
        4 & Spectral &  & 13.02 & 0.67 & 0.0 & 0.68 & 0.94 & 56.39 & 57.2 & 55.97 & 56.08 \\
        4 & Spectral & x & 14.52 & 0.16 & 0.0 & 0.27 & 3.11 & 56.29 & 56.14 & 56.44 & 56.35 \\				
	\end{tabular}
	\caption{$\sigma$ is the mean of all cluster price standard deviations, $\Delta_\mu$ is the average distance between cluster mean prices, $\Delta_{\text{min}}$ is the mean nearest neighbour cluster distance, $\Delta_{\text{avg}}$ denotes the average distance between all points situated in different clusters, and $DB$ is the Davies-Bouldin index. $DB$ has values in $[0, \infty)$ and measures the average similarity of every cluster with its most similar cluster. A low $DB$ index indicates a good clustering. $\mu_i$ denotes the mean price of cluster $i$. All metrics were computed considering the yearly average price for each node.}
	\label{tab:one-day}
\end{table}


